Quantum Shadow Gradient Descent for Variational Quantum Algorithms

Gradient-based optimizers have been proposed for training variational quantum circuits in settings such as quantum neural networks (QNNs). The task of gradient estimation, however, has proven to be challenging, primarily due to distinctive quantum features such as state collapse and measurement incompatibility. Conventional techniques, such as the parameter-shift rule, necessitate several fresh samples in each iteration to estimate the gradient due to the stochastic nature of state measurement. Owing to state collapse from measurement, the inability to reuse samples in subsequent iterations motivates a crucial inquiry into whether fundamentally more efficient approaches to sample utilization exist. In this paper, we affirm the feasibility of such efficiency enhancements through a novel procedure called quantum shadow gradient descent (QSGD), which uses a single sample per iteration to estimate all components of the gradient. Our approach is based on an adaptation of shadow tomography that significantly enhances sample efficiency. Through detailed theoretical analysis, we show that QSGD has a significantly faster convergence rate than existing methods under locality conditions. We present detailed numerical experiments supporting all of our theoretical claims.

==> App_numerical.tex <==
\noindent\textbf{Experiment 2:}
The second dataset is procedurally generated to classify between \textit{separable} and \textit{maximally entangled} states. To do this, we randomly generate several $2$-qubit density operators of the two different types. Separable states are of the form $\rho_A\tensor \rho_B$, where $\rho_A$ and $\rho_B$ each are single-qubit density operators ($2\times 2$ matrices) generated randomly based on a Haar measure using \textit{RandomDensityMatrix} in \citep{qetlab}. Each maximally entangled state is of the form $\ket{\psi}:=\frac{1}{4} (\ket{00}+\ket{01}+\ket{10}+\ket{11}).$ For the labeling, we assign $y=-1$ to separable states and $y=1$ to maximally entangled states. %The ansatz for this experiment is the same as in \eqref{eq:QNN exp}.


==> CST.tex <==
%\subsection{Quantum Shadow Sampling}\label{subsec:shadow}
 

\subsection{Shadow Gradient Estimation}\label{subsec:shadow gradient}

We construct an estimate of the gradient of the loss based on the created shadows. %Two alternative methods are considered. The first method keeps the shadow as a quantum state in a \ac{QC}. Then, it estimates the gradient by measuring the state using an appropriately designed measurement. The second method, which is the focus of this paper, 
Since, the shadow has a complete classical description, as it is generated from a classical outcome ($b_j$), one can directly compute the gradient of the loss on the shadows. %This approach converges faster than the first proposal, but at the cost of higher computational complexity. 
%{\bf ayg: I am not sure I understood the first method.}
In what follows, we provide a closed form expression for the gradient of the loss with respect to the shadows. 
%We now describe the procedure for direct computation of the gradient from the shadows. Note that, ideally we need $\nabla \Loss(\overrightarrow{a},\ket{\phi_t}, y_t)$ to apply the update rule \eqref{eq:QSGD ideal}. However, this quantity is unknown, since the input state is unknown.  Instead, we propose an estimate of the gradient based on the shadowing technique. 
%For that, we first study the gradient of the loss and derive its closed-form expression. 

We start by noting that $\nabla \Loss$ depends on the ansatz parametrization $U(\overrightarrow{a})$.

We consider two generic fomulations of the ansatz. The first formulation, which has been used widely in the literature, is a unitary operator defined as the product 
\begin{align}\label{eq:ansatz Pauli product}
U(\overrightarrow{a}) := \prod_{\ell=1}^k e^{ia_{\bfs_\ell} \sigma^{\bfs_\ell} },
\end{align}
where $\bfs\in \set{0,1,2,3}^d$ and $\sigma^{\bfs_\ell}$ is the $d$-fold tensor products of Pauli operators associated with $\bfs_\ell$.

We proceed with the following lemma which was used in \citep{HeidariAAAI2022}. For completeness the proof is given in Appendix \ref{proof:lem:loss derivative}.
\begin{lem}\label{lem:loss derivative}
Let ${\rho}^{out}_t =U(\overrightarrow{a}) \ketbra{\phi_t} U^\dagger(\overrightarrow{a})$ denote the density operator of the output state when the input to ansatz is $\ket{\phi_t}$. Then, the derivative of the loss is given by: 
\begin{align}\label{eq:losss derivative}
\frac{\partial  \Loss( \overrightarrow{a}, \ket{\phi_t}, y_t)}{\partial \qas} = \sum_{\hat{y}} i \ell(y_t,\hat{y})  \tr{M_{\hat{y}} \big[ \qps, {\rho}_t^{out}\big]},
\end{align}
where $[\cdot, \cdot]$ is the commutator operation.
\end{lem}

==> FullyQuantumQSGD.tex <==
\section{Fully Quantum Gradient Estimator}
\begin{itemize}
\item Computing the shadows is hard on classical computer. We perform everything on a QC.
\end{itemize}


\subsection{Unbiased Derivative Measurement}
 We now present a procedure for measuring the derivative of the expected loss (Figure \ref{fig:QNN gradient}). %Instead of approximating the derivative using the finite difference method, we compute it exactly using a method similar to that of Mitarai et al.~\cite{Mitarai2018}.  
  %
 The corresponding unitary operator can be written as: 
\begin{align}\label{eq:perceptron U1}
U(\overrightarrow{a}) = \exp\Big\{i\sum_{\bfs} \qas \qps \Big\},
\end{align}
where $\qps$ are the corresponding Pauli operators. 
In what follows, we intend to measure the derivative of the loss w.r.t. $\qas$ for a given $\bfs$ appearing in the summation above. In our method, at each time $t$, we apply the QNN on the $t^{th}$ sample $\rho_t$, which produces $\rho_t^{out}$. Next, we add an auxiliary qubit to $\rho^{out}_t$, which creates the following state:
 \begin{align}\label{eq:rho tild}
 \tilde{\rho}_t = \rho^{out}_t \tensor \ketbra{+}_E,
 \end{align}
 where $\ket{+}_E=\frac{1}{\sqrt{2}}(\ket{0}_E+\ket{{1}}_E)$, and $E$ represents the auxiliary Hilbert space. Then, we apply the following unitary operator on $\tilde{\rho}_t$:
 \begin{align}\label{eq:Vs}
 V_\bfs =  e^{i\frac{\pi}{4} \qps} \tensor \ketbra{0}_E + e^{-i\frac{\pi}{4} \qps} \tensor \ketbra{1}_E.
 \end{align}


\begin{figure}[tp]
\centering
\includegraphics[scale=1]{Figures/GradientQNN2.eps}
\caption{The procedure for measuring the derivative of the loss consisting of a unitary operator $V_\bfs$ followed by a quantum measurement $\mathcal{N}$ with additional classical processing. %is used to output a random variable $z_t=-2(-1)^by_t$.
}
\label{fig:QNN gradient}
\end{figure}

Next, we measure the state by a quantum measurement $\mathcal{N}:=\set{\Lambda_{b,\hat{y}}: \hat{y}\in \mathcal{Y}, b\in \{0,1\}}$ with outcomes in $\mathcal{Y}\times \{0,1\}$ and operators:
\begin{align}\label{eq:POVM N}
\Lambda_{b, \hat{y}}  = M_{\hat{y}} \tensor \ketbra{b}_E, \qquad \forall \hat{y}\in \mathcal{Y},~ b =0,1. 
\end{align}
Finally, if the outcome of this measurement is $(\hat{y},b)$, we compute $z_t =-2(-1)^b \ell(y,\hat{y})$ as the measured gradient, where $\ell(\cdot,\cdot)$ is the loss function. Note that $Z_t$ is a random variable depending on the current parameters of the network and the input sample  $(\rho_t, y_t)$. The following lemma,  shows that $Z_t$ is an unbiased measure of the derivative of loss with respect to $\qas$.  

\begin{lem}\label{lem:gradient estimation}
Let $Z_t$ be the output of the procedure shown in Figure \ref{fig:QNN gradient} applied on the $t^{th}$ sample. Then $Z_t$ is an unbiased estimate of the derivative of the loss. More precisely,  
$\EE[Z_t|y_t, \rho_t] = \frac{\partial \Loss( \overrightarrow{a}, \rho_t, y_t)}{\partial a}.$
\end{lem}

==> Notation_header.tex <==
%========================================================================================
%------------------------- This header contains shorthands and notations ----------------
%========================================================================================
\newcommand{\prodin}{\prod_{i=1}^n}
\newcommand{\sumin}{\sum_{i=1}^n}

%====================== double script fonts  =====================================

\global\long\def\RR{\mathbb{R}}
\global\long\def\CC{\mathbb{C}}
\global\long\def\NN{\mathbb{N}}
\global\long\def\QQ{\mathbb{Q}}
\global\long\def\ZZ{\mathbb{Z}}
\global\long\def\EE{\mathbb{E}}
\global\long\def\PP{\mathbb{P}}
\global\long\def\FF{\mathbb{F}}
\global\long\def\11{\mathbbm{1}}

%====================== math bold fonts  =====================================
\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

\newcommand{\clA}{\mathcal{A}}
\newcommand{\clC}{\mathcal{C}}
\newcommand{\clJ}{\mathcal{J}}
\newcommand{\clU}{\mathcal{U}}
\newcommand{\clV}{\mathcal{V}}
\newcommand{\clX}{\mathcal{X}}
\newcommand{\clY}{\mathcal{Y}}


%====================== shortcuts for operators  =====================================

\global\long\def\+{\oplus}
\global\long\def\P{\mathsf{P}}
\global\long\def\dd{\cdots}
\newcommand\pmm{\{-1,1\}}

\newcommand{\prob}[1]{\PP\Big\{  #1 \Big\} }
\def\<{\langle}
\def\>{\rangle}

%\newcommand{\sign}{\mathsf{sign}}
\DeclareMathOperator*{\sign}{sign}
\newcommand{\OR}{\mathsf{OR}}
\newcommand{\AND}{\mathsf{AND}}
\newcommand{\MAJ}{\mathsf{MAJ}}

\ifdefined \var 
  \renewcommand{\var}{\mathsf{var}}
\else
  \newcommand{\var}{\mathsf{var}}
\fi

\ifdefined \abs \else
 \newcommand{\abs}[1]{\lvert#1\rvert}
\fi

\ifdefined \norm \else
 \newcommand{\norm}[1]{\lVert#1\rVert}
\fi


\ifdefined \set 
  \renewcommand{\set}[1]{\left\{#1\right\}}
\else
  \newcommand{\set}[1]{\left\{#1\right\}}
\fi


\DeclareMathOperator*{\supp}{supp}

\newcommand*{\medcap}{\mathbin{\scalebox{1}{\ensuremath{\bigcap}}}}%
\newcommand*{\medcup}{\mathbin{\scalebox{1}{\ensuremath{\bigcup}}}}%
\newcommand*{\medprod}{\mathbin{\scalebox{1}{\ensuremath{\prod}}}}%

\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}

%-------- delta = for definition -----
\usepackage{stackengine}
%\def\deq{\mathrel{\ensurestackMath{\stackon[1pt]{=}{\scriptstyle\Delta}}}}
\def\deq{:=}
%===============================================================================
%------------------------- Special Notations -----------------------------------
%===============================================================================

%++++++++++++++++++++++++   Quantum Symbols ++++++++++++++++++++++++++++++++++++
\DeclareMathOperator*{\tensor}{\otimes}

%\DeclareMathOperator{\tr}{tr}
% \newcommand{\Tr}[1]{\lVert#1\rVert}

\providecommand{\tr}{tr}

\ifdefined \Tr 
  \renewcommand{\Tr}[1]{\tr \Big\{#1\Big\}}
\else
  \newcommand{\Tr}[1]{\tr \Big\{#1\Big\}}
\fi


 \def\id{I_d}
\global\long\def\bigtensor{\bigotimes}
\def\fy{\emph{F}_Y}
\def\gm{\emph{G}_M}
\def\gmA{\emph{G}_M^{\mathcal{A}}}
%+++++++++++++++++++ Quantum Fourier Learning Symbls ++++++++++++++++++++++++++
\def\qgs{{g}_{\bfs}}
\def\qYJ{\emph{F}_Y^{\mathcal{J}}}
\def\qYA{\emph{F}_Y^{\mathcal{A}}}
%\def\qYk{\emph{F}_Y^{\leq k}}
\def\qYk{{\emph{F}}_Y^{~k}}

\def\qfs{f_{\bfs}}
\def\qfests{\hat{f}_{\bfs}}

\def\qms{M_{\bfs}}


\def\qps{\sigma^\bfs}
\def\qfY{\emph{F}_{Y}}
\def\qfYest{{\hat{F}}}
\def\qfYestk{\hat{\emph{F}}_Y^{k}}
\def\qfsest{\hat{f}_{\bfs}}
\def\qfYestJ{{\qfYest}^{\mathcal{J}}}

\def\Msopt{\Lambda^{\bfs}}

\newcommand{\opt}{\optfont{opt}}
\def\Loss{L_{0-1}}

\def\BJ{B_{\mathcal{J}}}
\def\hJ{\BJ}
\def\PiJ{\Pi^{\mathcal{J}}}
\def\GJ{G_{\mathcal{J}}}
\def\PiJhat{{\hat{\Pi}}^{\mathcal{J}}}

%++++++++++++++++++++++++   Fourier Learning Symbls ++++++++++++++++++++++++++

\def\fS{{f}_{\mathcal{S}}}
\def\fJ{f^{\subseteq \mathcal{J}}}
\def\fd{f_{\Hspaced}}

\def\fJstar{{f}^{\subseteq {\mathcal{J}^*}}}
%\def\hJ{h_{\mathcal{J}}}

\def\gS{\tilde{g}_{\mathcal{S}}}
\def\gJ{g^{\subseteq J}}

\def\ps{\psi_\mathcal{S}}
\def\pS{\ps}

%++++++++++++++++++++++++   Esimation Symbls ++++++++++++++++++++++++++++++++++++
\def\festS{\hat{f}_{ S} }
\def\festJ{\hat{f}^{\subseteq \mathcal{J}}}

\def\fbarS{\bar{f}_{ S} }
\def\fbarJ{\bar{f}^{\subseteq \mathcal{J}}}


%\def\FestS{\hat{\mathsf{F}}_{S} }
\def\FestS{\festS}

%\def\FestJ{\hat{\mathsf{F}}^{\subseteq \mathcal{J}}}
\def\FestJ{\festJ}

\def\FestSone{\hat{f}_{(1), S} }
\def\FestJone{\hat{f}_{(1)}^{\subseteq \mathcal{J}}}
\def\FestJi{\hat{f}_{(i)}^{\subseteq \mathcal{J}}}

\def\pestS{\widehat{\psi}_{\mathcal{S}}}
\def\PestS{\widehat{\Psi}_{\mathcal{S}}}





%++++++++++++++++++++++++   Algorithm Symbls ++++++++++++++++++++++++++++++++++++

\def\Jalg{\hat{\mathcal{J}}}
\def\falg{\hat{f}^{\subseteq \Jalg}}
\def\fJalg{{f}^{\subseteq \Jalg}}

\def\predict{\hat{g}}
\def\Peg{P_e(\predict)}
\def\Pegb{P_e(\predict_2)}

\def\Jalgb{\hat{\mathcal{J}}_2}
\def\falgb{\hat{f}^{\subseteq \Jalgb}}
\def\fJalgb{{f}^{\subseteq \Jalgb}}
\def\predictb{\hat{g}_2}





\def\rndJalg{\mathscr{J}_{alg1}}
\def\rndfalg{\mathsf{F}_{est}^{\subseteq \rndJalg}}
\def\rndpredict{\mathsf{G}_{alg1}}
\def\frndJalg{{f}^{\subseteq \rndJalg}}



%\newcommand{\barf}{\bar{f}}
 \def\fbarJ{\bar{f}^{\subseteq J}}
\def\fJbar{f^{\subseteq \bar{J}}}
%\def\fbarJbar{\bar{f}^{\subseteq \bar{J}}}
%\def\festJbar{{f}_{est}^{\subseteq \bar{J}}}
%\def\fbarS{\bar{f}_{S} }
%\def\funivJbstar{{f}_{unv}^{\subseteq {\bar{J}^*}}}
%\def\funivJ{{f}_{unv}^{\subseteq {J}}}
%\def\Je{\mathcal{J}_{\mathbf{e}}}
%\def\E_mu{\mathcal{E}(\epsilon')}


\def\L2{\mathcal{L}^2(\mathcal{X}^d, P_{X^d})}
\def\Pspace{(\mathcal{X},P_{\bfX})}




\newcommand{\optfont}[1]{\mathsf{#1}}
%\newcommand{\Pek}{\optfont{P^k}[f]}
\newcommand{\Popt}{\opt_{k}}
\newcommand{\Pek}{\Popt}


\def\score{\operatorname{score}}
\def\imscore{{\score}}

\def\E_mu{\mathcal{E}_{\mu}(\epsilon')}
\def\Hspaced{\mathcal{H}_d}
\def\Hspacek{\mathcal{H}_k}

==> Proof_thm_shadow.tex <==
Given this string, we prepare $d$ qubits as $\ket{\omega^\Phi_j} :=V_j\ket{b^\Phi_j}, j\in [d]$.
%Let $\Gamma_0: \mathcal{B}[\mathcal{H}_2] \rightarrow \mathcal{B}[\mathcal{H}_2]$ be a linear mapping on $\mathcal{B}[\mathcal{H}_2]$, the space of all operators on the two dimensional Hilbert space $\mathcal{H}_2$. 
For any single-qubit operator $B$, define: 
% For any operator $\rho$ on the two dimensional Hilbert space, define: %{\bf ayg: is the Hilbert space two dimensional now or is it a power of two?}
\begin{align*}
 \Gamma_0[B]:=\hspace{-10pt}\sum_{V\in \set{ I, H, S^\dagger H}}\sum_{b\in \set{0,1}} \frac{1}{3}\matrixelement{b}{V^{\dagger} B V}{b}~ V\ketbra{b}V^\dagger.
 \end{align*} 
 When $d=1$, applying $\Gamma_0^{-1}$ gives single-qubit shadows \cite{Huang2020}. However, it can also be used in a parallel form for $d$-qubit shadow generation. Specifically, consider applying $\Gamma_0^{-1}$ on each qubit as: 
\begin{align}\label{eq:rho hat shadow}
\hat{\Psi}_{classical}: = \bigotimes_{j=1}^d \Gamma_0^{-1}\big[\ketbra{\omega^\Phi_j}\big].
\end{align}
 Surprisingly, even though this  process operates independently on each qubit, it creates an unbiased shadow even when the state is entangled across the $d$ qubits. %{\bf ayg: I'm not sure 
The classical shadows can be copied and used to estimate the expected output of several observables. The estimation is done via direct calculation of the relevant trace quantities \cite{Huang2020}. However, the use of classical computations makes the process prohibitive in large dimensions. In this work, we propose a procedure for generating quantum shadows.  
 %Note that the shadow $\hat{\Phi}$ is stochastic, since $b^\Phi$ and $V$ are random. 
 %Moreover, note that $\hat{\rho}$ can be copied several times without violating the no-cloning as $b$ is classical. 
 % To summarize, the flow of this procedure is depicted below: 
 % \begin{equation*}
 %     \ket{\psi}\rightarrow V\ket{\psi} \rightarrow b^\psi \rightarrow \ket{b^\psi}\rightarrow \ket{\omega^\psi}\rightarrow \hat{\rho}^\psi
 % \end{equation*}
  We proceed with deriving a closed-form characterization of $\Gamma_0$.
\begin{lem}\label{lem:gamma0 inverse}
For a generic state $\ket{\bfa}=a_0 \ket{0}+a_1\ket{1}$, we have that: 
\begin{align*}
\Gamma_0^{-1}[\ketbra{\bfa}] = \begin{bmatrix}
2|a_0|^2-|a_1|^2 & 3a_0a_1^*\\
3a_0^*a_1 & 2|a_1|^2-|a_0|^2
\end{bmatrix}.
\end{align*}
\end{lem}
The proof is provided in the Supplementary material.  Note that each $\ket{\omega^\Psi_j}$ belongs to the set $\set{\ket{0}, \ket{1}, \ket{+}, \ket{-}, \ket{+i}, \ket{-i}}$. For any $c\in \set{0,1,+,-,+i, -i}$, let $\bar{c}$ denote its basis complement. That is, if $c=0$ then $\bar{c}=1$; if  $c=+$, then $\bar{c}=-$, and if $c=+i$, then $\bar{c}=-i$.   Hence, from Lemma \ref{lem:gamma0 inverse}, applying $\Gamma_0^{-1}$ on $\ket{\omega^\Psi_j}$ gives:
\begin{align*}
&\Gamma_0^{-1}[\ketbra{\omega^\Phi_j}]=2\ketbra{\omega^\Phi_j}-\ketbra{\bar{\omega}^\Phi_j}.
%&\Gamma_0^{-1}[\ketbra{0}]=2\ketbra{0}-\ketbra{1},  & &\Gamma_0^{-1}[\ketbra{1}]=2\ketbra{1}-\ketbra{0}\\
%&\Gamma_0^{-1}[\ketbra{+}]=2\ketbra{+}-\ketbra{-},  & &\Gamma_0^{-1}[\ketbra{-}]=2\ketbra{-}-\ketbra{+}\\
%&\Gamma_0^{-1}[\ketbra{+i}]=2\ketbra{+i}-\ketbra{-i},&  &\Gamma_0^{-1}[\ketbra{-i}]=2\ketbra{-i}-\ketbra{+i}.
\end{align*}

Note that by normalizing the above expression, we obtain the mixed state: $\frac{2}{3}\ketbra{\omega^\Phi_j}-\frac{1}{3}\ketbra{\bar{\omega}^\Phi_j}$. Consider the following stochastic map (classical channel) on any $\omega \in \set{0,1,+,-,+i, -i}$:
%\[
%\hat{\Psi}_j : = \frac{2}{3}\ketbra{c_j}-\frac{1}{3}\ketbra{\bar{c}_j}.
%\]
%Once this process is done for every qubit, the output is $\hat{\Psi} = \tensor_{j=1}^d \hat{\Psi}_j$. 
%Alternatively we can perform the following maps: 
%Lets index $\set{ I, H, S^\dagger H}$ with  $\set{0,1,2},$ respectively.  If $\alpha_j$ is the index of the chosen unitary for the $j$th qubit, and $b_j^{\Psi}\in \set{0,1}$ is the measurement outcome, then we output
\begin{align*}
 Q[\omega] =  \begin{cases}
  (\omega, 1) & \text{with prob.} \frac{2}{3}\\
     (\bar{\omega}, -1) & \text{with prob.} \frac{1}{3}.
  \end{cases}
  \end{align*} 
We use $Q$ to generate the quantum shadows. The first component of the output is used to generate a qubit, while the second component is used as a weight during the gradient estimation process.   We apply  $Q[\omega^\Phi_j]$ for each $j\in [d]$ to get a pair $(c_j,w_j)$, where $c_j\in \set{0,1,+,-,+i, -i}$ and $w_j\in \pmm$ is the weight (see Fig. \ref{fig:stochastic QSS}).
%Note that given the choice of the unitary $V_j\in \set{ I, H, S^\dagger H}$ and the measurement outcome $b_j\in \set{0, 1}$, we can uniquely identify $\omega_j\in \set{0,1,+,-,+i, -i}$. For example, if $V_j=H$ and $b_j=0$, then $\omega_j=+$. Then,  
Next,  we prepare the state $\ket{c_j}$. Hence, we obtain the following state and the weight value:  
\begin{align}\label{eq:stochastic QSS}
 \hat{\Phi}:=\ketbra{c_1, c_2, \cdots, c_d}, \qquad  \hat{w}=\prod_{j=1}^d w_j.
 \end{align} 

==> derivative_circuit.tex <==
\begin{quantikz}
 \lstick{$\ket{\psi}$}&\gate{U_{\leq l}} &\gate{R_{\bfs_l}}&\qw  &\gate{R_{\bfs_l}} &\qw & \gate{U_{>l}} & \meter{} \arrow[r]&\rstick{$\hat{y}$}\\
 \lstick{$\ket{0}$} &\gate{H} &\ctrl{-1}  &\gate{X}& \ctrl{-1}  & \gate{X}& \qw & \meter{} \arrow[r]&\rstick{b}
\end{quantikz}

==> figures_import.tex <==
  \begin{figure*}[ht!]
  \captionsetup[subfigure]{justification=centering}
  \centering
  \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(mohseni)RQSGD_data_mohseni_0.72.pdf}
       % \caption {RQSGD, Exp. 1 %with $\eta_t=0.72/\sqrt{t}$
  %      } %\\ on Mohseni dataset}
      %  \label{subfig:M2}
        
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(mohseni)Approx_data_mohseni_0.08.pdf}
        % \caption {QSGD, Exp. 1 %with $\eta_t=0.08/\sqrt{t}$
        % } % \\ on Mohseni dataset}
        % \label{subfig:M1}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(mohseni)Exact_data_mohseni_0.7.pdf}
        % \caption {Exact Exp. 1% with $\eta_t=0.7/\sqrt{t}$
        % } %\\ on Mohseni dataset}
        % \label{subfig:M3}    
\end{subfigure}


\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(entanglement)RQSGD_data_entangled_0.72.pdf}
        % \caption {Randomized QSGD Exp. 2% with $\eta_t=0.72/\sqrt{t}$
        % } %\\ on Entanglement dataset}
         % \label{subfig:E2}        
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(entanglement)Approx_data_entangled_0.1.pdf}
        % \caption {QSGD, Exp. 2, product% with $\eta_t=0.1/\sqrt{t}$
        % } %\\ on Entanglement dataset}
        % \label{subfig:E1}    
  \end{subfigure}
\begin{subfigure}{0.3\textwidth}
                \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(entanglement)Exact_data_entangled_0.3.pdf}
                % \caption {Exact gradient on Exp. 2% with $\eta_t=0.3/\sqrt{t}$
                % } %\\ on Entanglement dataset}
                % \label{subfig:E3}
\end{subfigure}



\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(1DM_GHZ__single_perceptron)RQSGD__0.96.pdf}
        % \caption {RQSGD, Exp. 3% with $\eta_t=0.96/\sqrt{t}$
        % } % \\ on GHZ dataset}
       % \label{subfig:G2}       
\end{subfigure}
     \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(1DM_GHZ__perceptron)Approx__0.1.pdf}
        % \caption {QSGD, Exp. 3% with $\eta_t=0.1/\sqrt{t}$
        % } %\\ on GHZ dataset}
        % \label{subfig:G1}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(1DM_GHZ__single_perceptron)Exact__0.9.pdf}
        % \caption {Exact Exp. 3% with $\eta_t=0.9/\sqrt{t}$
        % } %\\ on GHZ dataset}
        % \label{subfig:G3}        
\end{subfigure}








  % \begin{subfigure}{0.25\textwidth}
  %       \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa entnglement)Approx_data_entangled_0.01.pdf}
  %       \caption {Shadow QGD on Exp. 2 prod% with $\eta_t=0.01/\sqrt{t}$
  %       } %\\ on Entanglement dataset}
  %       \label{subfig:E1}
  % \end{subfigure}
 
% \begin{subfigure}{0.245\textwidth}
%        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa_GHZ)Approx__0.01.pdf}
%        % \caption {QSGD, Exp. 3, product% with $\eta_t=0.01/\sqrt{t}$
%        % } %\\ on GHZ dataset}
%        % \label{subfig:G1}
% \end{subfigure}

  


% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Isolet.eps}
% % }  
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Covertype.eps}
% % } 
%     % \subfigure{
%     %     \includegraphics[scale=0.18]{figures/E1.eps}
%     %     \label{subfig:E1}
%     %     }

% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/E2.eps}
% %          \label{subfig:E2}
% % }

% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/USPS.eps}
% %  		}
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Australian.eps}
% % }
% \begin{subfigure}{0.3\textwidth}
%         \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(1DM_GHZ__perceptron)Approx__0.1.pdf}
%         \caption {Shadow QGD on Exp. 3 with $\eta_t=0.1/\sqrt{t}$} %\\ on GHZ dataset}
%         \label{subfig:G1}
% \end{subfigure}
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Isolet.eps}
% % }  


 
% \begin{subfigure}{0.245\textwidth}
%         \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa mohseni)Exact_data_mohseni_0.32.pdf}
%         % \caption {Exact Exp. 1, prod% with $\eta_t=0.32/\sqrt{t}$
%         % } %\\ on Mohseni dataset}
%         % \label{subfig:M3}
% \end{subfigure}
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Covertype.eps}
% % }

% \begin{subfigure}{0.245\textwidth}
%        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa_GHZ)Exact__0.1.pdf}
%        % \caption {Exact Exp. 3, prod% with $\eta_t=0.1/\sqrt{t}$
%        % } %\\ on GHZ dataset}
%        % \label{subfig:G3}      
% \end{subfigure}

% % \begin{subfigure}{0.9\textwidth}
% \centering
%         \includegraphics[scale=0.6]{figures/title3.pdf}
% \end{subfigure}

 \caption{Comparing the training loss in three experiments based on three methods: QSGD (this work), RQSGD \cite{HeidariAAAI2022}, and the ideal method using the exact gradient computation. The vertical axis is the training loss and the horizontal line is the training batches each containing 100 samples. The solid red lines are the expected loss, the blue dots are the empirical loss, and the black dashed line is the theoretical lower bound on the loss based on the Holevo-Helstrom theorem \citep{Holevo2012}. }
       % \vspace{-1 em}
    \label{fig:loss}
    % \vspace{-2 em}
\end{figure*} 


==> figures_import_product_ansatz.tex <==
  \begin{figure*}[ht!]
  \captionsetup[subfigure]{justification=centering}
  \centering
  \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa mohseni)RQSGD_data_mohseni_0.2.pdf}
        % \caption {Randomized QSGD on Exp. 1% with $\eta_t=0.2/\sqrt{t}$
        % } %\\ on Mohseni dataset}
        % \label{subfig:M2}
\end{subfigure}
  \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa mohseni)Approx_data_mohseni_0.009.pdf}
        % \caption {Shadow QGD on Exp. 1 %with $\eta_t=0.009/\sqrt{t}$
        % } % \\ on Mohseni dataset}
        % \label{subfig:M1}
\end{subfigure}
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Isolet.eps}
% % }  
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/Covertype.eps}
% % }
\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa mohseni)Exact_data_mohseni_0.32.pdf}
        % \caption {Exact gradient on Exp. 1% with $\eta_t=0.32/\sqrt{t}$
        % } %\\ on Mohseni dataset}
        % \label{subfig:M3}   
\end{subfigure}

\begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa entnglement)RQSGD_data_entangled_0.2.pdf}
        % \caption {Randomized QSGD Exp. 2% with $\eta_t=0.2/\sqrt{t}$
        % } %\\ on Entanglement dataset}
        %  \label{subfig:E2}        
\end{subfigure}
  \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa entnglement)Approx_data_entangled_0.01.pdf}
        % \caption {Shadow QGD on Exp. 2% with $\eta_t=0.01/\sqrt{t}$
        % } %\\ on Entanglement dataset}
        % \label{subfig:E1}    
  \end{subfigure}
%     % \subfigure{
%     %     \includegraphics[scale=0.18]{figures/E1.eps}
%     %     \label{subfig:E1}
%     %     }
% %     \subfigure{
% %         \includegraphics[scale=0.18]{figures/E2.eps}
% %          \label{subfig:E2}
% % }
\begin{subfigure}{0.3\textwidth}
                \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa entnglement)Exact_data_entangled_0.2.pdf}
                % \caption {Exact gradient on Exp. 2% with $\eta_t=0.2/\sqrt{t}$
                % } %\\ on Entanglement dataset}              
                % \label{subfig:E3}              
\end{subfigure}

\begin{subfigure}{0.3\textwidth}
       \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa_GHZ)RQSGD__0.35.pdf}
       % \caption {Randomized QSGD on Exp. 3 with $\eta_t=0.35/\sqrt{t}$} % \\ on GHZ dataset}
       % \label{subfig:G2}
 \end{subfigure}
\begin{subfigure}{0.3\textwidth}
       \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa_GHZ)Approx__0.01.pdf}
       % \caption {Shadow QGD on Exp. 3 with $\eta_t=0.01/\sqrt{t}$} %\\ on GHZ dataset}
       % \label{subfig:G1}
\end{subfigure}
\begin{subfigure}{0.3\textwidth}
       \includegraphics[width=\textwidth]{Figures/SummaryOutcome/(pa_GHZ)Exact__0.1.pdf}
       % \caption {Exact gradient on Exp. 3 with $\eta_t=0.1/\sqrt{t}$} %\\ on GHZ dataset}
       % \label{subfig:G3}      
\end{subfigure}


% \begin{subfigure}{0.9\textwidth}
% \centering
%         \includegraphics[scale=0.6]{figures/title3.pdf}
% \end{subfigure}

    \caption{The training loss comparison with product ansatz. % Comparing the training loss in two experiments based on three methods using product ansatz: shadow QGD (this work), Randomized QSGD, and the ideal method using the exact gradient computation. The vertical axis is the training loss and the horizontal line is the training batches each containing 100 samples. 
   % The solid red lines are the expected loss, the blue dots are the empirical loss, and the black dashed line is the theoretical lower bound on the loss based on the Holevo-Helstrom theorem \citep{Holevo2012}. 
    }
       % \vspace{-1 em}
    \label{fig:loss products}
    % \vspace{-2 em}
\end{figure*} 


==> proof_lem_shadow.tex <==
\section{Proof of Lemma \ref{lem:shadow unbiased}}\label{appx:prop_Fourier_correlated}

{\bf ayg: Fix broken reference of lemma number} 

\begin{customlemma}{\ref{lem:shadow unbiased}}
Let $\hat{\rho}$ be the created shadow as in \eqref{eq:rho hat shadow} when the input is $\rho$. Then, $\EE[\hat{\rho}]=\rho$. 
\end{customlemma}

\begin{proof}
Let $V_j, j\in [d]$ be the selected unitary operators. Let $\bfV=\tensor_j V_j$. Recall from \eqref{eq:rho hat shadow} in the main text that:
\begin{align*}
\hat{\rho}:=\bigotimes_{j=1}^d \Gamma_0^{-1}\big[\ketbra{\omega^\rho_j}\big],
\end{align*}
where $\ket{\omega^\rho_j}= V_j\ket{b_j}$.
Let $P_\bfb$ denote the probability that the outcome of the measurement in the shadow sampling is $\bfb\in \set{0,1}^d$. Then, conditioned on the choice of $V_j$'s we have:  
\begin{align*}
P_\bfb &= \expval{\bfV \rho \bfV^\dagger}{\bfb}.
\end{align*}
Note that $V_j$'s are chosen randomly and uniformly from the set $\set{ I, H, S^\dagger H}$. Therefore, taking the expectation of $\hat{\rho}$ over the choice of $\bfV$ and the distribution $P_\bfb$ gives: 
\begin{align*}
   \EE[\hat{\rho}] &= \sum_{\bfb}P_\bfb   \sum_{V_j, j\in [d]} \frac{1}{3^d} \bigotimes_{j=1}^d \Gamma_0^{-1}\big[V_j\ketbra{b_j}V_j^\dagger\big]\\\numberthis \label{eq:E hat rho}
   &= \sum_{\bfb}P_\bfb  \bigotimes_{j=1}^d \Big( \sum_{V_j} \frac{1}{3} \Gamma_0^{-1}\big[V_j\ketbra{b_j}V_j^\dagger\big]\Big),
\end{align*}
where we used the fact that the terms inside the tensor product run independently.
It is known that any operator like $\rho$ has a Pauli decomposition of the form $\rho = \sum_{\bfs} \alpha_\bfs \qps,$ where $\qps$'s are $d$-fold tensor products of Pauli operators and $\alpha_\bfs= 2^{-d}\tr{\rho \qps}$ \citep{Montanaro2008}. As a result, we have:
\begin{align*}
    P_\bfb &=  \sum_{\bfs} \alpha_\bfs\expval{\bfV \qps \bfV^\dagger}{\bfb} \\
    & = \sum_{\bfs} \alpha_\bfs\prod_{j} \expval{V_j \sigma^{s_j} V_j^\dagger}{b_j}.
\end{align*}
Plugging this in \eqref{eq:E hat rho} gives
\begin{align*}
   \EE[\hat{\rho}] &= \sum_{\bfs} \alpha_\bfs  \bigotimes_{j=1}^d \Big( \sum_{b_j, V_j}\frac{1}{3}\expval{V_j \sigma^{s_j} V_j^\dagger}{b_j}   \Gamma_0^{-1}\big[V_j\ketbra{b_j}V_j^\dagger\big]\Big)\\
   &\stackrel{(a)}{=}\sum_{\bfs} \alpha_\bfs  \bigotimes_{j=1}^d \Gamma_0^{-1}\Big[ \sum_{b_j,V_j}\frac{1}{3}\expval{V_j \sigma^{s_j} V_j^\dagger}{b_j}   V_j\ketbra{b_j}V_j^\dagger\Big]\\
   &\stackrel{(b)}{=}\sum_{\bfs} \alpha_\bfs  \bigotimes_{j=1}^d \Gamma_0^{-1}\Big[\Gamma_0[\sigma^{s_j}] \Big]\\
   &\stackrel{(c)}{=}\sum_{\bfs} \alpha_\bfs  \bigotimes_{j=1}^d\sigma^{s_j}.
\end{align*}
where (a) follows from the linearity of $\Gamma_0^{-1}$, (b) follows from the definition of $\Gamma_0$, and (c) follows from the fact that $\Gamma_0^{-1}$ is the inverse of $\Gamma_0$.%Since  is a linear mapping, then so is its tensor products as in \eqref{eq:rho hat shadow} in the main text. Therefore, the Pauli decomposition of $\rho$ together with the linearity of $\Gamma_0^{-1}$  imply that  $\hat{\rho} = \sum_{\bfs} \alpha_s \Psi[\qps]$. %Since, $\qps$ is in tensor product and $\Psi$ operates on each qubit independently, $\Psi[\qps] = \tensor_{j=1}^d \Psi_j[\sigma^{s_j}]$, where $\Psi_j$ is the $j$th wire in Figure \ref{fig:Shadow dqubit}. As a result, 
  From this equation, we prove that $\EE[\hat{\rho}] = \sum_{\bfs} \alpha_s  \qps = \rho$, which completes the proof.
\end{proof}







==> proof_thm2.tex <==
\begin{proof}
Let $\overrightarrow{V}_t = \widehat{\nabla \Loss}(\parameter,\hat{\rho}^{out}_t, Y_t)$ be a sequence of random vectors
Theorem 14.8 of \citep{Shalev2014}, stats that 
Let $f$ be a convex function and $w^* = \argmin_{w:\norm{w}\leq B} f(w)$. Let $\{\overrightarrow{V}_t\}_{t=1}^T$ be a sequence of random vectors from SGD satisfying $\EE[\overrightarrow{V}_t | w^{(t)}] = \nabla f(w^{(t)})$, and $\norm{V_t}\leq \alpha$ with probability 1 for all $t$. Then, running SGD for $T$ iterations with $\eta = \frac{B}{\alpha \sqrt{T}}$ gives the following inequality 
\begin{align*}
\EE[f(w_{ave})] - f(w^*) \leq \frac{B\alpha}{\sqrt{T}},
\end{align*}
where $w_{ave} = \frac{1}{T}\sum_t w^{(t)}.$
%\end{customthm}
As a result, from Theorem 1 of the main paper, setting $\overrightarrow{V}_t=c_{QNN}\overrightarrow{Z}_t$ gives a sequence of random vectors satisfying $\EE[\overrightarrow{V}_t| \rho_t, y_t]= \nabla \Loss(\overrightarrow{a},\rho_t, y_t)$. Since component of $\overrightarrow{Z}_t$ are zero except at one coordinate taking values from $-2(-1)^{b}\ell(y, \hat{y})$, then 
\begin{align*}
\norm{V_t} \leq c_{QNN} \norm{\overrightarrow{Z}_t} \leq 2 \gamma c_{QNN} ,
\end{align*}
where $\gamma = \max_{y,\hat{y}} \abs{\ell(y, \hat{y})}.$ Consequently, the proof is complete by applying the above theorem with $B=1$ and $\alpha = 2 \gamma c_{QNN}$. 
\end{proof}


==> proof_thm_convergence.tex <==
\section{Proof of Theorem \ref{thm:convex QSGD}}\label{proof:thm:convex QSGD}
\begin{customthm}{\ref{thm:convex QSGD}}

{\bf ayg: fix broken ref}

Assume that the expected loss $\Loss(\overrightarrow{a})$ is a convex function of $\overrightarrow{a}$ and that loss function $\ell(y, \hat{y})$ is bounded from above by $\gamma>0$. Let $\overrightarrow{a}^* = \argmin_{\overrightarrow{a}: \|{\overrightarrow{a}}\| = 1}\Loss(\overrightarrow{a})$. If shadow QGD (Algorithm \ref{alg:QSGD}) is performed on $n$ \ac{iid} samples with $\eta_t = \frac{1}{ \gamma\sqrt{n}}$, then: $$
\EE[\Loss(\overrightarrow{a}_{ave})]- \Loss(\overrightarrow{a}^*) \leq \frac{\gamma }{\sqrt{n}},$$
%\end{align*}
where $\overrightarrow{a}_{ave} = \frac{1}{n}\sum_t \overrightarrow{a}^{(t)}$. 
\end{customthm}

 Our proof starts with the following lemma: 
\begin{customlemma}{\ref{lem:shadow gradient unbiased}}
Shadow gradient is an unbiased estimate of the gradient. That is, 
$$\EE[\widehat{\nabla \Loss}(\parameter,\hat{\rho}^{out}_t, y_t)]=\nabla \Loss(\parameter,\ket{\phi_t}, y_t),$$
for any sample $(\ket{\phi_t}, y_t)$, and parameter $\parameter$. Here, the expectation is taken with respect to the underlying randomness in the generation of the shadow $\hat{\rho}^{out}_t$. 
\end{customlemma}
\begin{proof}[Proof of Lemma \ref{lem:shadow gradient unbiased}]
Taking the expectation of each $g_\bfs$ in \eqref{eq:shadow derivative} gives:
\begin{align*}
    \EE[g_\bfs]= \sum_{\hat{y}} i \ell(y_t,\hat{y})  \tr{M_{\hat{y}} \EE\Big[\big[ \qps, \hat{\rho}_t^{out}\big]\Big]},
\end{align*}
where we use linearity of the expectation and the trace. Linearity of the commutator implies that:
\begin{align*}
    \EE\Big[\big[ \qps, \hat{\rho}_t^{out}\big]\Big] &= \qps \EE[\hat{\rho}_t^{out}] - \EE[\hat{\rho}_t^{out}] \qps,
    \end{align*}
Lemma \ref{lem:shadow unbiased} implies that $\EE[\hat{\rho}_t^{out}] = {\rho}_t^{out},$ where ${\rho}_t^{out}=U(\overrightarrow{a})\ketbra{\phi_t} U^\dagger(\overrightarrow{a})$ is the true output state. Therefore, the above expectation equals $\big[ \qps, {\rho}_t^{out}\big]$. Hence, with Lemma \ref{lem:loss derivative}, we obtain that $\EE[g_\bfs]$ gives the same expression as in \eqref{eq:losss derivative}, which is the true derivative of the loss. Hence, we proved that $\EE[\widehat{\nabla \Loss}]=\nabla \Loss$, as desired. 
\end{proof}

%Our numerical results demonstrate the convergence of randomized QSGD for training QNNs. 
%    We note here that, similar to the classical NNs, the convexity requirement is not generally satisfied in QNNs. However, our analysis with the convexity assumption provides insights on the convergence rate even for non-convex (DNN) objective functions solved using trust region, cubic regularization, or related techniques. Our numerical results in the next section demonstrate the convergence of randomized QSGD for training QNNs. 

With this lemma and taking expectation over the randomness in training sample generation, we obtain the following equality:
 $$\EE_{(\ket{\phi_t}, Y_t)\sim D}\Big[\EE[\widehat{\nabla \Loss}(\parameter,\hat{\rho}^{out}_t, Y_t) \big| \ket{\phi_t}, Y_t]\Big] = \nabla \Loss(\parameter).$$
 Using this relation and standard analysis of classical SGD  \cite{Shalev2014}, we obtain our convergence result. The formal proof of the theorem follows.   
%

%\input{proof_thm2.tex} 

Denote ${W}_t = \widehat{\nabla \Loss}(\parameter,\hat{\rho}^{out}_t, Y_t)$ for all $t=1,2,..., n$. Note that from the above equation, $\{{W}_t\}_{t\geq 1}$ forms a sequence of random vectors satisfying $\EE[{W}_t | \parameter^{(t)}] = \nabla \Loss(\parameter^{(t)})$ for all $t\geq 1$. Moreover, since $\ell$ is bounded by $\gamma$, then $|W_t|\leq \gamma$ almost surely for all $t\geq 1$. With these conditions, we can apply Theorem 14.8 of \citep{Shalev2014} on the convergence of classical SGD for convex functions. Here, the cost function is $\Loss(\parameter)$ and $V_t$'s are the sub-gradients. Consequently with $\eta_t = \frac{1}{\gamma \sqrt{n}}$, we obtain the desired  inequality: 
\begin{align*}
\EE[\Loss(\overrightarrow{a}_{ave})]- \Loss(\overrightarrow{a}^*) \leq \frac{\gamma }{\sqrt{n}},
\end{align*}
which completes the proof.
%\end{proof}

==> proof_thm_trotter.tex <==
\section{Proof of Theorem \ref{thm:loss derivative non product}}
\begin{customthm}{\ref{thm:loss derivative non product}}
For a non-prodct ansatz $U(\overrightarrow{a})$ as in \eqref{eq:ansatz Pauli}, let $\rho^{out}$ be the output state. For any $\bft\in \set{0,1,2,3}^d$, define $\frac{\partial \tilde{\Loss}}{\partial a_\bft}:=\sum_{\hat{y}} i \ell(y,\hat{y})  \tr{M_{\hat{y}} \big[ \sigma^\bft, {\rho}^{out}\big]}$, where $y$ is the true label.  Then, the derivative of the loss for the non-product $U$ expands in terms of  $\frac{\partial \tilde{\Loss}}{\partial a_\bft}$ as: 
 \begin{equation*}
     \frac{\partial\Loss}{\partial a_\bfs} = \frac{\partial \tilde{\Loss}}{\partial a_\bfs}+ \sum_{\bfr, \bft} {a}_{\bfr}(\kappa_{\bfr \bfs \bft}-\kappa_{\bfs \bfr \bft})  \frac{\partial \tilde{\Loss}}{\partial a_{\bft}} + \frac{1}{3}\sum_{\bfr, \bfq, \bfr', \bft}  a_{\bfr}a_{\bfr'}  \kappa_{\bfr \bfs \bfq} \kappa_{\bfq \bfr' \bft}   \frac{\partial \tilde{\Loss}}{\partial a_{\bft}}, \qquad \forall \bfs\in \set{0,1,2,3}^d.  % \sum_{\bfs''}  \sum_{\substack{\bfs'\leq  \bfr':\\ \bfs'  \circ \bfs\circ \bfr' = \bfs'' }} a_{\bfs'}a_{\bfr'} \frac{\partial \tilde{\Loss}}{\partial a_{\bfs''}},  
 \end{equation*}
  %for any $\bfs\in \set{0,1,2,3}^d$.
\end{customthm}
\begin{proof}
Let $W_n:= \prod_{\bfs} \exp{i\frac{\qas}{n}\qps}.$ Then from Theorem 3 of \cite{Suzuki1976}, 
\begin{align*}
U(\parameter) = \lim_{n\rightarrow \infty} W_n^n.
\end{align*}
The derivative of the loss with respect to $\qas$ is 
\begin{align*}
\frac{\partial \Loss}{\partial \qas} = \sum_{\hat{y}} \ell(y, \hat{y}) \tr{M_{\hat{y}}\frac{\partial }{\partial \qas}\Big(U(\parameter)\rho U^\dagger(\parameter)\Big) }.
\end{align*}
Since the derivative of $W_n$ is a converging sequence, we can  interchange  limit with the derivative. operator:
\begin{align*}
\frac{\partial \Loss}{\partial \qas} =  \lim_{n\rightarrow \infty}\sum_{\hat{y}} \ell(y, \hat{y}) \tr{M_{\hat{y}}\frac{\partial }{\partial \qas}\Big(W_n^n\rho W_n^{n \dagger}\Big) }.
\end{align*}
Consider an ordering of the elements of $\set{0,1,2,3}^d$ and define the following operators
\begin{align*}
W_{\leq \bfs}:= \prod_{\bfs' < \bfs} \exp{i \frac{a_{\bfs'}}{n}\sigma^{\bfs'}}, \qquad W_{\geq \bfs}:= \prod_{\bfs' \geq \bfs} \exp{i\frac{a_{\bfs'}}{n}\sigma^{\bfs'}}
\end{align*}
With this notation, the derivative of $W_n$ equals to the following
\begin{align*}
\tilde{W}_n:= \frac{\partial W_n}{\partial \qas} = \frac{i}{n}W_{< \bfs}\sigma^{\bfs} W_{\geq \bfs}
\end{align*}
Then the derivative of $W_n^n$ equals to 
\begin{align*}
\frac{\partial W_n}{\partial \qas} = \sum_{k=0}^{n-1} W_n^k \tilde{W} W_n^{n-k-1}.
\end{align*}
As a result, we have that 
\begin{align*}
\frac{\partial }{\partial \qas}\Big(W_n^n\rho W_n^{n \dagger}\Big) &= \Big(\frac{\partial W_n^n }{\partial \qas}\Big) \rho W_n^{n \dagger} + W_n^n \rho \Big(\frac{\partial W_n^{n \dagger} }{\partial \qas}\Big)\\
&=  \sum_{k}W_n^k \tilde{W} W_n^{n-k-1} \rho W_n^{n \dagger} -  \sum_{k}W_n^n \rho W_n^{k\dagger} \tilde{W}^\dagger W_n^{n-k-1 \dagger}\\
&= \sum_{k}W_n^k \tilde{W} W_n^{n-k-1} \rho W_n^{n \dagger} - W_n^n \rho W_n^{n-k-1\dagger} \tilde{W}^\dagger W_n^{k \dagger},
\end{align*}
where the last inequality follows by changing $k$ to $n-k-1$ in the second summation. Let $\rho_{n}^{out}: = W_n^n\rho W_n^{n\dagger}$. Then, from the above expression and by noting that $W_n^{k+1}W_n^{k+1\dagger}=I$ we have that 
\begin{align*}
\frac{\partial }{\partial \qas}\Big(W_n^n\rho W_n^{n \dagger}\Big) &= \sum_{k} W_n^k \tilde{W} W_n^{k+1\dagger} \rho_{n}^{out} - \rho_{n}^{out}  W_n^{k+1} \tilde{W}^\dagger W_n^{k \dagger},
  \end{align*} 
  
Define $A_{n, k}: = W_n^k W_{< \bfs}$. Then, we have that 
\begin{align*}
W_n^k \tilde{W} W_n^{k+1\dagger}&=\frac{i}{n}W_n^k W_{< \bfs}\sigma^{\bfs} W_{\geq \bfs} W_n^{k+1\dagger}\\
&= A_{n, k} \sigma^{\bfs}A_{n,k}^\dagger.
 \end{align*} 
As a result the above derivative equals to 
\begin{align}\label{eq:loss derivative 1}
\frac{\partial \Loss}{\partial \qas} = \lim_{n\rightarrow \infty}\frac{i}{n} \sum_{\hat{y}} \ell(y, \hat{y}) \sum_{k} \tr{M_{\hat{y}} [A_{n, k} \sigma^{\bfs}A_{n,k}^\dagger, \rho_n^{out}]}.
\end{align}
Next, we apply Taylor's approximation as 
\begin{align*}
\exp{i\frac{a_{\bfs'}}{n}\sigma^{bfs'}} = I+i\frac{a_{\bfs'}}{n}\sigma^{\bfs'} + \order{\frac{1}{n^2}}. 
\end{align*}
Then, we can write 
\begin{align*}
W_n = \prod_{\bfs'} \Big(I+i\frac{a_{\bfs'}}{n}\sigma^{\bfs'} + \order{\frac{1}{n^2}}\Big)=I+i\sum_{\bfs'}\frac{a_{\bfs'}}{n}\sigma^{\bfs'} + \order{\frac{c}{n^2}},
\end{align*}
where $c$ is the number of the parameters $\qas$, and we used the fact that $\sum_\bfs |\qas|^2 = O(c)$.  
Rising both sides to the power $k$ and using the inequality $(1+x)^k =1+kx +O(x^2)$ on the right-hand side give 
\begin{align*}
W^k_n = I+ik \sum_{\bfs'}\frac{a_{\bfs'}}{n}\sigma^{\bfs'} + \order{\frac{kc}{n^2}}.
\end{align*}
Similarly, using the Taylor;s expansion for each term in $W_{< \bfs}$, we get $$W_{<\bfs} = I+ \frac{i}{n}\sum_{\bfs'' <\bfs} a_{\bfs''} \sigma^{\bfs''} + \order{\frac{c}{n^2}}.$$ 
Therefore, we can write $A_{n,k}$ as
\begin{align*}
A_{n,k} = W_n^k W_{< \bfs} &=  I+\frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\sigma^{\bfs'} + \frac{i}{n}\sum_{\bfs'' <\bfs} a_{\bfs''} \sigma^{\bfs''}+ \order{\frac{kc}{n^2}}.
\end{align*}
Consequently, we have that 
\begin{align*}
A_{n,k}\rho_n^{out}A_{n,k}^\dagger &=\qps + \frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\sigma^{\bfs'} \qps +\frac{i}{n}\sum_{\bfs'' <\bfs} a_{\bfs''} \sigma^{\bfs''} \qps -\frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\qps \sigma^{\bfs'} - \frac{i}{n}\sum_{\bfs'' <\bfs} a_{\bfs''} \qps \sigma^{\bfs''}\\
& + \frac{k^2}{n^2} \sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'}\sigma^{\bfs'} \qps \sigma^{\bfr'} +\frac{1}{n^2}\sum_{\bfs'', \bfr'' <\bfs} a_{\bfs''}a_{\bfr''} \sigma^{\bfs''} \qps \sigma^{\bfr''}\\
&+\frac{k}{n^2} \sum_{\substack{\bfs'\\ \bfr''<\bfs}}a_{\bfs'}a_{\bfr''}\sigma^{\bfs'} \qps \sigma^{\bfr''} +\frac{k}{n^2} \sum_{\substack{\bfs''<\bfs,\\ \bfr'}}a_{\bfs''}a_{\bfr'}\sigma^{\bfs''} \qps \sigma^{\bfr'}+\order{\frac{kc}{n^2}}. 
\end{align*}
Note that the third, fifth, seventh, eighth and ninth are bounded be a corresponding big-O notation as 
\begin{align*}
A_{n,k}\rho_n^{out}A_{n,k}^\dagger &=\qps + \frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\sigma^{\bfs'} \qps + \order{\frac{c}{n}}-\frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\qps \sigma^{\bfs'}+\order{\frac{c}{n}}\\
&+ \frac{k^2}{n^2} \sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'}\sigma^{\bfs'} \qps \sigma^{\bfr'}+\order{\frac{c^2}{n^2}}+\order{\frac{kc^2}{n^2}}+\order{\frac{kc^2}{n^2}}+\order{\frac{kc}{n^2}}\\
&=\underbrace{\qps}_{(I)} + \underbrace{\frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\sigma^{\bfs'} \qps}_{(II)} -\underbrace{\frac{ik}{n} \sum_{\bfs'}a_{\bfs'}\qps \sigma^{\bfs'}}_{(III)} +  \underbrace{\frac{k^2}{n^2} \sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'}\sigma^{\bfs'} \qps \sigma^{\bfr'}}_{(IV)}+\order{\frac{c}{n}+\frac{kc^2}{n^2}}.
 \end{align*} 
 Plugging this into \eqref{eq:loss derivative 1} gives
 \begin{align*}
\frac{\partial \Loss}{\partial \qas} = \lim_{n\rightarrow \infty}\frac{i}{n} \sum_{\hat{y}} \ell(y, \hat{y}) \sum_{k}\tr{M_{\hat{y}} [(I)+(II)+(III)+(IV), \rho_n^{out}]} + \Delta,
 \end{align*}
 where $\Delta$ is the residual term given by
 \begin{align*}
\Delta =  \lim_{n\rightarrow \infty}\frac{\ell^{max}}{n} \sum_k \order{\frac{c}{n}+\frac{kc^2}{n^2}},
 \end{align*}
 where used the fact that $|\ell(y, \hat{y})| \leq \ell^{max}<\infty$, and that $\sum_{\hat{y}}M_{\hat{y}}=I$ due to the POVM formulation. This residual term is equal to zero, because 
 \begin{align*}
 \Delta =  \lim_{n\rightarrow \infty}\frac{\ell^{max}}{n}    \order{c+\frac{n(n+1)c^2}{2n^2}} =\lim_{n\rightarrow \infty} \order{\frac{\ell^{max}c}{n}+\frac{\ell^{max} (n+1)c^2}{2n^2}} =0.
 \end{align*}
 Hence, it remains to compute the main terms. 
 \paragraph{(I):} 
 \begin{align*}
 \lim_{n\rightarrow \infty}\frac{i}{n} \sum_{\hat{y}} \ell(y, \hat{y}) \sum_{k}\tr{M_{\hat{y}} [\qps, \rho_n^{out}]} &=  \lim_{n\rightarrow \infty}i \sum_{\hat{y}} \ell(y, \hat{y})\tr{M_{\hat{y}} [\qps, \rho_n^{out}]}\\
 &=i\sum_{\hat{y}} \ell(y, \hat{y}) \tr{M_{\hat{y}} [\qps, \Big( \lim_{n\rightarrow \infty}\rho_n^{out}\Big)]}\\
&=  i\sum_{\hat{y}} \ell(y, \hat{y}) \tr{M_{\hat{y}} [\qps, \rho^{out}]} = \frac{\partial \tilde{\Loss}}{\partial \qas}
 \end{align*}
  \paragraph{(II):} 
  \begin{align*}
  \lim_{n\rightarrow \infty}&\sum_{\bfs'}a_{\bfs'}  \sum_{\hat{y}} \ell(y, \hat{y}) \sum_{k}\frac{-k}{n^2} \tr{M_{\hat{y}}  [ \sigma^{\bfs'} \qps, \rho_n^{out}]}=  \lim_{n\rightarrow \infty}\sum_{\bfs'}a_{\bfs'}  \sum_{\hat{y}} \ell(y, \hat{y}) \frac{-n(n+1)}{2n^2} \tr{M_{\hat{y}}  [ \sigma^{\bfs'} \qps, \rho_n^{out}]}\\
  & = -\frac{1}{2}\sum_{\bfs'}a_{\bfs'}  \sum_{\hat{y}} \ell(y, \hat{y}) \tr{M_{\hat{y}}  [ \sigma^{\bfs'} \qps, \lim_{n\rightarrow \infty} \frac{(n+1)}{n}\rho_n^{out}]}\\
  &= -\frac{1}{2}\sum_{\bfs'}a_{\bfs'}  \sum_{\hat{y}} \ell(y, \hat{y}) \tr{M_{\hat{y}}  [ \sigma^{\bfs'} \qps, \rho^{out}]}.
  \end{align*}
  Next, from the definition of $\kappa_{jk\ell}$ we can write,  $\sigma^{\bfs'} \qps= \sum_{\bft}  \kappa_{\bfs',\bfs,\bft} \sigma^\bft$.  Hence, from the definition of $\frac{\partial \tilde{\Loss}}{\partial \qas }$ the term (II) equals to $ -\frac{1}{2}\sum_{\bfs', \bft}a_{\bfs'} \kappa_{\bfs',\bfs,\bft}\frac{\partial \tilde{\Loss}}{\partial a_{\bft}}$.
  
  
  \paragraph{(III):} This is similar to the previous part and simplifies to $ \frac{1}{2}\sum_{\bfs', \bft}a_{\bfs'} \kappa_{\bfs,\bfs',\bft}\frac{\partial \tilde{\Loss}}{\partial a_{\bft}}$.
  
  
  \paragraph{(IV):}
  \begin{align*}
  \lim_{n\rightarrow \infty}&\sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'} \sum_{\hat{y}} \ell(y, \hat{y}) \sum_k \frac{k^2}{n^2}   \tr{M_{\hat{y}}  [ \sigma^{\bfs'} \qps \sigma^{\bfr'}, \rho_n^{out}]}\\
  & =  \lim_{n\rightarrow \infty}\sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'} \sum_{\hat{y}} \ell(y, \hat{y}) \frac{n(n+1)(2n+1)}{6n^3}   \tr{M_{\hat{y}}  [ \sigma^{\bfs'} \qps \sigma^{\bfr'}, \rho_n^{out}]}\\
  & =  \sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'} \sum_{\hat{y}} \ell(y, \hat{y})    \tr{M_{\hat{y}}  [\sigma^{\bfs'} \qps \sigma^{\bfr'}, \Big( \lim_{n\rightarrow \infty} \frac{(n+1)(2n+1)}{6n^2} \rho_n^{out}\Big)]} \\
  & =  \sum_{\bfs', \bfr'}a_{\bfs'}a_{\bfr'} \sum_{\hat{y}} \ell(y, \hat{y})    \tr{M_{\hat{y}}  [\sigma^{\bfs'} \qps \sigma^{\bfr'}, \rho^{out}]}.
   \end{align*}
   Note that $\sigma^{\bfs'} \qps\sigma^{\bfr'} = \sum_{\bfq, \bft}  \kappa_{\bfs' \bfs \bfq} \kappa_{\bfq \bfr' \bft}\sigma^{\bft}.$ Hence, the derivative related to the $(IV)$ term equals to $\frac{1}{3}\sum_{\bfr, \bfq, \bfr', \bft}  a_{\bfr}a_{\bfr'}  \kappa_{\bfr \bfs \bfq} \kappa_{\bfq \bfr' \bft}   \frac{\partial \tilde{\Loss}}{\partial a_{\bft}}$.
   
Combining all the terms proves the theorem. 
\end{proof}
